Propositions in Linear Multirole Logic as Multiparty Session Types

We identify multirole logic as a new form of logic and formalize linear multirole logic (LMRL) as a natural generalization of classical linear logic (CLL). Among various meta-properties established for LMRL, we obtain one named multi-cut elimination stating that every cut between three (or more) sequents (as a generalization of a cut between two sequents) can be eliminated, thus extending the celebrated result of cut-elimination by Gentzen. We also present a variant of $\pi$-calculus for multiparty sessions that demonstrates a tight correspondence between process communication in this variant and multi-cut elimination in LMRL, thus extending some recent results by Caires and Pfenning (2010) and Wadler (2012), among others, along a similar line of work.

==> pgfutil-common-lists.tex <==
% Copyright 2013 by Christian Feuersaenger
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%5
%
% This list here is a general re-implementation of the list used in
% the PGF system layer.
% It employs two collect-buffers to reduce the runtime.
%
% - It has preasymptotical runtime O(N), but is O(N^2) asymptotically.
% - It requires only 5 macros per list.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Usage: 
% \pgfapplistnewempty\macro
\def\pgfapplistnewempty#1{%
	\expandafter\let\csname pgfapp@#1\endcsname=\pgfutil@empty
	\expandafter\let\csname pgfapp@#1@smallbuf\endcsname=\pgfutil@empty
	\expandafter\let\csname pgfapp@#1@bigbuf\endcsname=\pgfutil@empty
	\expandafter\def\csname pgfapp@#1@smallbuf@c\endcsname{0}%
	\expandafter\def\csname pgfapp@#1@bigbuf@c\endcsname{0}%
}%

% #1: the item to append
% #2: the list as macro name
\long\def\pgfapplistpushback#1\to#2{%
	\begingroup
		\c@pgf@counta=\csname pgfapp@#2@smallbuf@c\endcsname\relax
		\advance\c@pgf@counta by1
		\xdef\pgf@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\expandafter\let\csname pgfapp@#2@smallbuf@c\endcsname=\pgf@glob@TMPa
	\ifnum\csname pgfapp@#2@smallbuf@c\endcsname<40
		\t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfapp@#2@smallbuf\endcsname#1}%
		\expandafter\edef\csname pgfapp@#2@smallbuf\endcsname{\the\t@pgf@toka}%
	\else
		\pgfapplistpushback@smallbufoverfl{#1}{#2}%
	\fi
}%
\long\def\pgfapplistpushback@smallbufoverfl#1#2{%
	\begingroup
		\c@pgf@counta=\csname pgfapp@#2@bigbuf@c\endcsname\relax
		\advance\c@pgf@counta by1
		\xdef\pgf@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\expandafter\let\csname pgfapp@#2@bigbuf@c\endcsname=\pgf@glob@TMPa
	%
	\ifnum\csname pgfapp@#2@bigbuf@c\endcsname<30
		\t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfapp@#2@bigbuf\endcsname}%
		\t@pgf@tokb=\expandafter\expandafter\expandafter{\csname pgfapp@#2@smallbuf\endcsname#1}%
		\expandafter\edef\csname pgfapp@#2@bigbuf\endcsname{\the\t@pgf@toka\the\t@pgf@tokb}%
		\expandafter\let\csname pgfapp@#2@smallbuf\endcsname=\pgfutil@empty
		\expandafter\def\csname pgfapp@#2@smallbuf@c\endcsname{0}%
	\else%
		\t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfapp@#2\endcsname}%
		\t@pgf@tokb=\expandafter\expandafter\expandafter{\csname pgfapp@#2@bigbuf\endcsname}%
		\t@pgf@tokc=\expandafter\expandafter\expandafter{\csname pgfapp@#2@smallbuf\endcsname#1}%
		\expandafter\edef\csname pgfapp@#2\endcsname{\the\t@pgf@toka\the\t@pgf@tokb\the\t@pgf@tokc}%
		\expandafter\let\csname pgfapp@#2@smallbuf\endcsname=\pgfutil@empty
		\expandafter\def\csname pgfapp@#2@smallbuf@c\endcsname{0}%
		\expandafter\let\csname pgfapp@#2@bigbuf\endcsname=\pgfutil@empty
		\expandafter\def\csname pgfapp@#2@bigbuf@c\endcsname{0}%
	\fi%
}%
\def\pgfapplist@flushbuffers#1{%
	\t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfapp@#1\endcsname}%
	\t@pgf@tokb=\expandafter\expandafter\expandafter{\csname pgfapp@#1@bigbuf\endcsname}%
	\t@pgf@tokc=\expandafter\expandafter\expandafter{\csname pgfapp@#1@smallbuf\endcsname}%
	\expandafter\edef\csname pgfapp@#1\endcsname{\the\t@pgf@toka\the\t@pgf@tokb\the\t@pgf@tokc}%
	\expandafter\let\csname pgfapp@#1@smallbuf\endcsname=\pgfutil@empty
	\expandafter\def\csname pgfapp@#1@smallbuf@c\endcsname{0}%
	\expandafter\let\csname pgfapp@#1@bigbuf\endcsname=\pgfutil@empty
	\expandafter\def\csname pgfapp@#1@bigbuf@c\endcsname{0}%
}%

\def\pgfapplistlet#1=#2{%
	\pgfapplist@flushbuffers{#2}%
	\expandafter\let\expandafter#1\csname pgfapp@#2\endcsname
}%
	

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 
% A variant of applist which has the same runtime requirements, but
% does PUSH FRONT only.
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% Usage: 
% \pgfprependlistnewempty{list}
\def\pgfprependlistnewempty#1{%
	\expandafter\let\csname pgfpPRP@#1\endcsname=\pgfutil@empty
	\expandafter\let\csname pgfpPRP@#1@smallbuf\endcsname=\pgfutil@empty
	\expandafter\let\csname pgfpPRP@#1@bigbuf\endcsname=\pgfutil@empty
	\expandafter\def\csname pgfpPRP@#1@smallbuf@c\endcsname{0}%
	\expandafter\def\csname pgfpPRP@#1@bigbuf@c\endcsname{0}%
}%

% #1: the item to append
% #2: the list as macro name
\long\def\pgfprependlistpushfront#1\to#2{%
	\begingroup
		\c@pgf@counta=\csname pgfpPRP@#2@smallbuf@c\endcsname\relax
		\advance\c@pgf@counta by1
		\xdef\pgf@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\expandafter\let\csname pgfpPRP@#2@smallbuf@c\endcsname=\pgf@glob@TMPa
	\ifnum\csname pgfpPRP@#2@smallbuf@c\endcsname<40
		\t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfpPRP@#2@smallbuf\endcsname}%
		\t@pgf@tokb={#1}%
		\expandafter\edef\csname pgfpPRP@#2@smallbuf\endcsname{\the\t@pgf@tokb\the\t@pgf@toka}%
	\else
		\pgfprependlistpushfront@smallbufoverfl{#1}{#2}%
	\fi
}%
\long\def\pgfprependlistpushfront@smallbufoverfl#1#2{%
	\begingroup
		\c@pgf@counta=\csname pgfpPRP@#2@bigbuf@c\endcsname\relax
		\advance\c@pgf@counta by1
		\xdef\pgf@glob@TMPa{\the\c@pgf@counta}%
	\endgroup
	\expandafter\let\csname pgfpPRP@#2@bigbuf@c\endcsname=\pgf@glob@TMPa
	%
	\ifnum\csname pgfpPRP@#2@bigbuf@c\endcsname<30
		\t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfpPRP@#2@bigbuf\endcsname}%
		\t@pgf@tokb=\expandafter\expandafter\expandafter{\csname pgfpPRP@#2@smallbuf\endcsname}%
		\t@pgf@tokc={#1}%
		\expandafter\edef\csname pgfpPRP@#2@bigbuf\endcsname{\the\t@pgf@tokc\the\t@pgf@tokb\the\t@pgf@toka}%
		\expandafter\let\csname pgfpPRP@#2@smallbuf\endcsname=\pgfutil@empty
		\expandafter\def\csname pgfpPRP@#2@smallbuf@c\endcsname{0}%
	\else%
		\pgfprependlist@flushbuffers{#2}%
		\t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfpPRP@#2\endcsname}%
		\t@pgf@tokb={#1}%
		\expandafter\edef\csname pgfpPRP@#2\endcsname{\the\t@pgf@tokb\the\t@pgf@toka}%
	\fi%
}%
\def\pgfprependlist@flushbuffers#1{%
	\t@pgf@toka=\expandafter\expandafter\expandafter{\csname pgfpPRP@#1\endcsname}%
	\t@pgf@tokb=\expandafter\expandafter\expandafter{\csname pgfpPRP@#1@bigbuf\endcsname}%
	\t@pgf@tokc=\expandafter\expandafter\expandafter{\csname pgfpPRP@#1@smallbuf\endcsname}%
	\expandafter\edef\csname pgfpPRP@#1\endcsname{\the\t@pgf@tokc\the\t@pgf@tokb\the\t@pgf@toka}%
	\expandafter\let\csname pgfpPRP@#1@smallbuf\endcsname=\pgfutil@empty
	\expandafter\def\csname pgfpPRP@#1@smallbuf@c\endcsname{0}%
	\expandafter\let\csname pgfpPRP@#1@bigbuf\endcsname=\pgfutil@empty
	\expandafter\def\csname pgfpPRP@#1@bigbuf@c\endcsname{0}%
}%
\def\pgfprependlistlet#1=#2{%
	\pgfprependlist@flushbuffers{#2}%
	\expandafter\let\expandafter#1\csname pgfpPRP@#2\endcsname
}%


==> pgfutil-common.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.


% 
% This file provides utitiliy commands that are used throughout pgf.
%
% For most commands, the definition of these commands is just given
% below. We cannot use the LaTeX definition of these commands since
% LaTeX may not be the current format and since LaTeX packages tend to
% redefine these commands.
%
% For some commands the actual definition of the format (like latex or
% context) is to be preferred over the generic definition below. In
% this case, the definition of the format is installed when the file
% pgfutil-XXXX.tex is read, where XXXX is the format name (latex,
% plain, or context). 



\catcode`\@=11\relax


% Which format is loaded?
\newif\ifpgfutil@format@is@latex
\newif\ifpgfutil@format@is@plain
\newif\ifpgfutil@format@is@context


% Simple stuff

% \pgfutil@ifundefined{<macro name with backslash>}
%  {<is undefined code>}{<is defined code>}
%
% This will let #1 to \relax if it undefined.
%
% This macro is expandable.
\def\pgfutil@ifundefined#1{%
  \expandafter\ifx\csname#1\endcsname\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi}

% A variant of \pgfutil@ifundefined which will NOT let #1 to \relax it
% is undefined. However, this macro is not expandable.
\def\pgfutil@IfUndefined#1{%
  \begingroup\expandafter\expandafter\expandafter\endgroup
  \expandafter\ifx\csname#1\endcsname\relax
    \expandafter\pgfutil@firstoftwo
  \else
    \expandafter\pgfutil@secondoftwo
  \fi
}
\long\def\pgfutil@firstofone#1{#1}
\long\def\pgfutil@firstoftwo#1#2{#1}
\long\def\pgfutil@secondoftwo#1#2{#2}
\def\pgfutil@empty{}
\def\pgfutil@gobble@until@relax#1\relax{}
\def\pgfutil@gobble#1{}
\def\pgfutil@gobbletwo#1#2{}
\def\pgfutil@namedef#1{\expandafter\def\csname #1\endcsname}
\def\pgfutil@namelet#1{\expandafter\pgfutil@@namelet\csname#1\endcsname}
\def\pgfutil@@namelet#1#2{\expandafter\let\expandafter#1\csname#2\endcsname}
\long\def\pgfutil@g@addto@macro#1#2{%
  \begingroup
    \pgfutil@toks@\expandafter{#1#2}%
    \xdef#1{\the\pgfutil@toks@}%
 \endgroup}
\newif\ifpgfutil@tempswa
\newif\ifpgfutil@tempswb

% pgfutil@ifnextchar

\long\def\pgfutil@ifnextchar#1#2#3{%
  \let\pgfutil@reserved@d=#1%
  \def\pgfutil@reserved@a{#2}%
  \def\pgfutil@reserved@b{#3}%
  \futurelet\pgfutil@let@token\pgfutil@ifnch}
\def\pgfutil@ifnch{%
  \ifx\pgfutil@let@token\pgfutil@sptoken
    \let\pgfutil@reserved@c\pgfutil@xifnch
  \else
    \ifx\pgfutil@let@token\pgfutil@reserved@d
      \let\pgfutil@reserved@c\pgfutil@reserved@a
    \else
      \let\pgfutil@reserved@c\pgfutil@reserved@b
    \fi
  \fi
  \pgfutil@reserved@c}
{%
  \def\:{\global\let\pgfutil@sptoken= } \:
  \def\:{\pgfutil@xifnch} \expandafter\gdef\: {\futurelet\pgfutil@let@token\pgfutil@ifnch}
}

% pgfutil@in@

\newif\ifpgfutil@in@

% Usage:
% \pgfutil@in@{one}{three two one}
% \ifpgfutil@in@
% 	-> will be true!
% \else
% \fi
%
% \pgfutil@in@{,}{1234,456567}
% \ifpgfutil@in@
% 	-> will be true!
% \else
% \fi
\def\pgfutil@in@#1#2{%
 \def\pgfutil@in@@##1#1##2##3\pgfutil@in@@{%
  \ifx\pgfutil@in@##2\pgfutil@in@false\else\pgfutil@in@true\fi}%
 \pgfutil@in@@#2#1\pgfutil@in@\pgfutil@in@@}


% pgfutil@for

\def\pgfutil@nnil{\pgfutil@nil}
\def\pgfutil@fornoop#1\@@#2#3{}
\long\def\pgfutil@for#1:=#2\do#3{%
  \expandafter\def\expandafter\pgfutil@fortmp\expandafter{#2}%
  \ifx\pgfutil@fortmp\pgfutil@empty \else
    \expandafter\pgfutil@forloop#2,\pgfutil@nil,\pgfutil@nil\@@#1{#3}\fi}
\long\def\pgfutil@forloop#1,#2,#3\@@#4#5{\def#4{#1}\ifx #4\pgfutil@nnil \else
       #5\def#4{#2}\ifx #4\pgfutil@nnil \else#5\pgfutil@iforloop #3\@@#4{#5}\fi\fi}
\long\def\pgfutil@iforloop#1,#2\@@#3#4{\def#3{#1}\ifx #3\pgfutil@nnil
       \expandafter\pgfutil@fornoop \else
      #4\relax\expandafter\pgfutil@iforloop\fi#2\@@#3{#4}}
\def\pgfutil@tfor#1:={\pgfutil@tf@r#1 }
\long\def\pgfutil@tf@r#1#2\do#3{\def\pgfutil@fortmp{#2}\ifx\pgfutil@fortmp\pgfutil@space\else
    \pgfutil@tforloop#2\pgfutil@nil\pgfutil@nil\@@#1{#3}\fi}
\long\def\pgfutil@tforloop#1#2\@@#3#4{\def#3{#1}\ifx #3\pgfutil@nnil
       \expandafter\pgfutil@fornoop \else
      #4\relax\expandafter\pgfutil@tforloop\fi#2\@@#3{#4}}

\def\pgfutil@space{ }

% pgfutil@IfFileExists

%\chardef\pgfutil@inputcheck0
\def\pgfutil@IfFileExists#1#2#3{%
  \openin\pgfutil@inputcheck=#1 %
  \ifeof\pgfutil@inputcheck
     #3\relax
  \else
    #2\relax
  \fi
  \closein\pgfutil@inputcheck}

\def\pgfutil@InputIfFileExists#1#2#3{\pgfutil@IfFileExists{#1}{\input #1\relax#2}{#3}}%


% pgfutil@loop (from plain.tex)

\def\pgfutil@loop#1\pgfutil@repeat{\def\pgfutil@body{#1}\pgfutil@iterate}
\def\pgfutil@iterate{\pgfutil@body \let\pgfutil@next\pgfutil@iterate \else\let\pgfutil@next\relax\fi \pgfutil@next}
\let\pgfutil@repeat=\fi % this makes \loop...\if...\repeat skippable


% aux-read-hook

\let\pgfutil@aux@read@hook=\relax


% Tokens for the end of the typesetting -- they will be added at the
% end of every job (hopefully...).

\newtoks\pgfutil@everybye


%
% PDF-Resource management -- might seem strange that this is here, but
% it turns out to be the correct place since latex and context handle
% this stuff quite differently
%

% Adding something to the pdf-resources:

\def\pgfutil@addpdfresource@extgs#1{\pgf@sys@addpdfresource@extgs@plain{#1}}
\def\pgfutil@addpdfresource@colorspaces#1{\pgf@sys@addpdfresource@colorspaces@plain{#1}}
\def\pgfutil@addpdfresource@patterns#1{\pgf@sys@addpdfresource@patterns@plain{#1}}
\def\pgfutil@setuppdfresources{\pgf@sys@setuppdfresources@plain}


% Inserts the argument at the begin of the current page (hopefully)

\let\pgfutil@insertatbegincurrentpage=\relax


% Ragged left and ragged right

\def\pgfutil@raggedright{\rightskip\z@ plus2em \spaceskip.3333em \xspaceskip.5em\relax}
\def\pgfutil@raggedleft{\leftskip\z@ plus2em \rightskip\z@ \spaceskip.3333em \xspaceskip.5em\parfillskip0pt\relax}


% Error Messages
\def\pgfutil@packageerror#1#2#3{\errhelp{#3}\errmessage{Package #1 Error: #2}}
\def\pgfutil@packagewarning#1#2{\immediate\write17{Package #1: Warning! #2.}}
\def\pgferror#1{\pgfutil@packageerror{pgf}{#1}{}}
\def\pgfwarning#1{\pgfutil@packagewarning{pgf}{#1}}


% Library files inclusion


% Include a library file.
%
% #1 = List of names of library file.
%  
% Description:
%
% This command includes a list of library files. For each file X in the
% list, the file pgflibraryX.code.tex is included, provided this has
% not been done earlier. 
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usepgflibrary{arrows}
% \usepgflibrary[patterns,snakes]

\def\usepgflibrary{\pgfutil@ifnextchar[{\use@pgflibrary}{\use@@pgflibrary}}%}
\def\use@pgflibrary[#1]{\use@@pgflibrary{#1}}
\def\use@@pgflibrary#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\pgfkeys@spdef\expandafter\pgf@temp\expandafter{\pgf@temp}%
    \ifx\pgf@temp\pgfutil@empty
    \else
      \expandafter\ifx\csname pgf@library@\pgf@temp @loaded\endcsname\relax%
      \expandafter\let\csname pgf@library@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname pgf@library@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname pgf@library@#1@barcode\endcsname{\the\catcode`\|}
      \expandafter\edef\csname pgf@library@#1@dollarcode\endcsname{\the\catcode`\$}
      \catcode`\@=11
      \catcode`\|=12
      \catcode`\$=3
      \pgfutil@InputIfFileExists{pgflibrary\pgf@temp.code.tex}{}{%
          \pgferror{I did not find the pgf library
            '\pgf@temp'. I looked for the file named
            pgflibrary\pgf@temp.code.tex, but could not find it in in
            the current texmf trees.} 
        }%
      \catcode`\@=\csname pgf@library@#1@atcode\endcsname
      \catcode`\|=\csname pgf@library@#1@barcode\endcsname
      \catcode`\$=\csname pgf@library@#1@dollarcode\endcsname
      \fi%
    \fi
  }%
}


% Include a module file.
%
% #1 = List of names of module files.
%  
% Description:
%
% This command includes a list of module files. For each file X in the
% list, the file pgfmoduleX.code.tex is included, provided this has
% not been done earlier. 
%
% For the convenience of Context users, both round and square brackets
% are possible for the argument.
%
% Example:
%
% \usepgfmodule{matrix}

\def\usepgfmodule{\pgfutil@ifnextchar[{\use@pgfmodule}{\use@@pgfmodule}}%}
\def\use@pgfmodule[#1]{\use@@pgfmodule{#1}}
\def\use@@pgfmodule#1{%
  \edef\pgf@list{#1}%
  \pgfutil@for\pgf@temp:=\pgf@list\do{%
    \expandafter\ifx\csname pgf@module@\pgf@temp @loaded\endcsname\relax%
      \expandafter\let\csname pgf@module@\pgf@temp @loaded\endcsname=\pgfutil@empty%
      \expandafter\edef\csname pgf@module@#1@atcode\endcsname{\the\catcode`\@}
      \expandafter\edef\csname pgf@module@#1@barcode\endcsname{\the\catcode`\|}
      \expandafter\edef\csname pgf@module@#1@dollarcode\endcsname{\the\catcode`\$}
      \catcode`\@=11
      \catcode`\|=12
      \catcode`\$=3
      \input pgfmodule\pgf@temp.code.tex
      \catcode`\@=\csname pgf@module@#1@atcode\endcsname
      \catcode`\|=\csname pgf@module@#1@barcode\endcsname
      \catcode`\$=\csname pgf@module@#1@dollarcode\endcsname
    \fi%
  }%
}

\def\pgfutilensuremath#1{%
  \ifmmode#1\else$#1$\fi
}


%
% Guess the driver:
%

\begingroup
	\catcode`\"=12
	\edef\pgf@loc@TMPa{"}%
	%
	% prepares file names by checking for double colons.
	%
	% If '#1' is a usual file name without anything fancy, \pgfretval
	% will simply contain it. However, if '#1' contains double colons
	% (introduces, for example, by pdftex because there are white
	% spaces in '#1'), the routine 
	% - removes the double colons,
	% - re-inserts them outside of the string.
	%
	% \pgfutilpreparefilename{file.tex} -> file.tex
	% \pgfutilpreparefilename{"A file name".file} -> "A file name.file"
	%
	% The resulting file name is returned in '\pgfretval',
	% furthermore, a *quoted* version of the file name is returned in
	% \pgfretvalquoted. The latter result is to have some sort of
	% output normalisation: if the file name as such contains double
	% quotes, we don't want to insert another set of them.
	%
	% This special handling has the following purposes:
	% 1. Both, treatment of white spaces and double colons is not
	% properly defined in TeX. Thus, we should only work with them if
	% necessary and maintain backwards compatibility as far as
	% possible.
	% 2. It *should* work if there are spaces.
	%
	\gdef\pgfutilpreparefilename#1{%
		\begingroup
			\ifnum\the\catcode`\"=13
				\pgfutilconvertdcolon
			\fi
			\xdef\pgf@temp{#1}%
		\endgroup
		\expandafter\pgfutil@in@\expandafter"\expandafter{\pgf@temp}%
		\ifpgfutil@in@
			\def\pgf@loc@TMPa{\pgfutilstrreplace{"}{}}%
			\expandafter\pgf@loc@TMPa\expandafter{\pgf@temp}%
			\edef\pgfretval{"\pgfretval"}% re-insert quotes! Otherwise, TeX can't use the file name.
			\let\pgfretvalquoted=\pgfretval
		\else
			\let\pgfretval=\pgf@temp
			\edef\pgfretvalquoted{"\pgfretval"}%
		\fi
	}%
	\catcode`\"=13
	\xdef\pgfutilconvertdcolon{%
		\noexpand\def\noexpand"{\pgf@loc@TMPa}%
	}%
\endgroup

% Usage:
% \pgfutilstrreplace{<token>}{<replacement>}{<string>}
%
% -> will assign the modified string into \pgfretval.
%
% #1: the string to search (one or more tokens)
% #2: zero, one or more tokens which will be inserted instead of '#1'.
% #3: the string to search in
\long\def\pgfutilstrreplace#1#2#3{%
	\def\pgfretval{}%
	\long\def\pgfutil@search@and@replace@@##1#1##2\pgf@EOI{%
		\expandafter\def\expandafter\pgfretval\expandafter{\pgfretval ##1#2}%
		\pgfutil@search@and@replace@loop{#1}{##2}%
	}%
	\pgfutil@search@and@replace@loop{#1}{#3}%
}
\long\def\pgfutil@search@and@replace@loop#1#2{%
	\pgfutil@in@{#1}{#2}%
	\ifpgfutil@in@
		\def\pgf@loc@TMPa{\pgfutil@search@and@replace@@ #2\pgf@EOI}%
	\else
		\expandafter\def\expandafter\pgfretval\expandafter{\pgfretval #2}%
		\let\pgf@loc@TMPa=\relax
	\fi
	\pgf@loc@TMPa
}%

% Solves a linear equation system of size 2x2 using gauss elimination.
%
% It employs TeX register arithmetics to do so.
% #1: should contain 4 sets of braces with matrix entries, 
% 	{<a11>}{<a12>}
% 	{<a21>}{<a22>}
% 	where each entry should be a number without unit.
% 	It is acceptable if '#1' is a macro which expands to the expected
% 	format.
% #2: should contain 2 sets of braces with the right-hand-side,
% 	{<r1>}{<r2>}
% 	where each entry should be a number without unit.
% 	It is acceptable if '#2' is a macro which expands to the expected
% 	format.
%
% It will assign \pgfmathresult to contain two sets of braces with the
% result.
%
% Example:
% \pgfutilsolvetwotwoleq{
% 	{0.24}{1}
% 	{-0.97}{0}
% }{
% 	{-7}
% 	{18}
% }
% -> yields \pgfmathresult={−18.55618}{−2.54642}
%
% The algorithm employs column pivotisation.
\def\pgfutilsolvetwotwoleq#1#2{%
	\begingroup
		\dimendef\aa=0
		\dimendef\ab=1
		\dimendef\ba=2
		\dimendef\bb=3
		\dimendef\ra=4
		\dimendef\rb=5
		\dimendef\tmpa=6
		\dimendef\tmpb=7
		\edef\pgf@temp{#1}%
		\expandafter\pgfutilsolvetwotwoleq@A\pgf@temp
		\edef\pgf@temp{#2}%
		\expandafter\pgfutilsolvetwotwoleq@r\pgf@temp
		%
		\pgfutilsolvetwotwoleq@ifislarger\aa\ba{%
			% identity "permutation":
			\def\Pa{a}%
			\def\Pb{b}%
		}{%
			% permutation matrix: switch rows!
			\def\Pa{b}%
			\def\Pb{a}%
		}%
		% \pivot := 1/aa
		\pgfmathreciprocal@
			{\csname m\Pa a\endcsname}%
		\let\pivot=\pgfmathresult
		%
		% \factor := 1/aa * ba 
		\csname \Pb a\endcsname=\pivot\csname \Pb a\endcsname
		\edef\factor{\expandafter\pgf@sys@tonumber\csname \Pb a\endcsname}%
		%
		% bb -= ba/aa * ab
		\tmpa=-\factor\csname \Pa b\endcsname
		\advance\csname \Pb b\endcsname by\tmpa
		%
		% rb -= ba/aa * ra
		\tmpa=-\factor\csname r\Pa\endcsname
		\advance\csname r\Pb\endcsname by\tmpa
		%
		% xb := rb / bb (the modified rb and modified bb!)
		\pgfmathdivide@
			{\expandafter\pgf@sys@tonumber\csname r\Pb\endcsname}
			{\expandafter\pgf@sys@tonumber\csname \Pb b\endcsname}%
		\expandafter\let\csname pgfmathresult\Pb\endcsname=\pgfmathresult
		%
		% ra -= xb * ab
		\tmpa=\csname pgfmathresult\Pb\endcsname\csname \Pa b\endcsname
		\advance\csname r\Pa\endcsname by-\tmpa
		%
		% xa := 1/aa * ra  (the modified ra!)
		\tmpa=\pivot\csname r\Pa\endcsname
		\expandafter\edef\csname pgfmathresult\Pa\endcsname{\pgf@sys@tonumber\tmpa}%
		%
		\edef\pgfmathresult{%
			{\csname pgfmathresult\Pa\endcsname}%
			{\csname pgfmathresult\Pb\endcsname}%
		}%
		\pgfmath@smuggleone\pgfmathresult
	\endgroup
}%
\def\pgfutilsolvetwotwoleq@ifislarger#1#2#3#4{%
	\tmpa=#1
	\ifdim\tmpa<0pt
		\multiply\tmpa by-1
	\fi
	\tmpb=#2
	\ifdim\tmpb<0pt
		\multiply\tmpb by-1
	\fi
	\ifdim\tmpa>\tmpb
		#3%
	\else
		#4%
	\fi
}%
\def\pgfutilsolvetwotwoleq@A#1#2#3#4{%
	\def\maa{#1}\def\mab{#2}%
	\def\mba{#3}\def\mbb{#3}%
	\aa=#1pt \ab=#2pt
	\ba=#3pt \bb=#4pt
}
\def\pgfutilsolvetwotwoleq@r#1#2{%
	\ra=#1pt \rb=#2pt
}%

% there are funny programs which overwrite \read and \write (like
% tabularx).
\let\pgfutil@write=\write
\let\pgfutil@read=\read

% curtesy for latex:
\let\pgfutil@protect\relax

% Used by latex for doing reruns
% #1 = an internal label
% #2 = a to-be-tested text 
\def\pgfutil@check@rerun#1#2{}

% new tempdims:
\newdimen\pgfutil@tempdima
\newdimen\pgfutil@tempdimb


% luatex stuff
% We assume luatex version > 0.39:
%   - \directlua <general text> will work
%   - \directlua is the only luatex primitive that we can assume
%     accessible without being prefixed by the format via
%     tex.enableprimitives.
% Ideas taken from the ifluatex package (Heiko Oberdiek)
\let\pgfutil@ifluatex\iffalse
\begingroup\expandafter\expandafter\expandafter\endgroup
\expandafter\ifx\csname directlua\endcsname\relax
\else
  \expandafter\let\csname pgfutil@ifluatex\expandafter\endcsname
    \csname iftrue\endcsname
\fi

\pgfutil@ifluatex
  \let\pgfutil@directlua\directlua
  \pgfutil@directlua{%
    tex.enableprimitives('pgfutil@',{'luaescapestring'})}
\else
  \def\pgfutil@directlua#1{}
  \def\pgfutil@luaescapestring#1{}
\fi
% End of luatex stuff

% Advances a number stored in a macro and writes the result back into
% the macro.
% #1 is a macro containing a number. 
\def\pgfutil@advancestringcounter#1{%
	\begingroup
		\c@pgf@counta=#1\relax
		\advance\c@pgf@counta by1
		\edef#1{\the\c@pgf@counta}%
		\pgfmath@smuggleone#1%
	\endgroup
}%
\input pgfutil-common-lists.tex

\endinput


==> tikzlibraryarrows.code.tex <==
% Copyright 2006 by Till Tantau
%
% This file may be distributed and/or modified
%
% 1. under the LaTeX Project Public License and/or
% 2. under the GNU Public License.
%
% See the file doc/generic/pgf/licenses/LICENSE for more details.

\ProvidesFileRCS[v\pgfversion] $Header: /cvsroot/pgf/pgf/generic/pgf/frontendlayer/tikz/libraries/tikzlibraryarrows.code.tex,v 1.1 2008/01/09 17:57:15 tantau Exp $

\usepgflibrary{arrows}

\endinput


==> xkeyval.tex <==
%%
%% This is file `xkeyval.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvtex')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2014 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvutils.tex, pst-xkey.tex, pst-xkey.sty, xkveca.cls,
%% xkvecb.cls, xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex,
%% xkvex2.tex, xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, xkvutils.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname XKeyValLoaded\endcsname
\let\XKeyValLoaded\endinput
\edef\XKVcatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \catcode`\noexpand\=\the\catcode`\=\relax
  \catcode`\noexpand\,\the\catcode`\,\relax
  \catcode`\noexpand\:\the\catcode`\:\relax
  \let\noexpand\XKVcatcodes\relax
}
\catcode`\@11\relax
\catcode`\=12\relax
\catcode`\,12\relax
\catcode`\:12\relax
\input xkvutils
\newcount\XKV@depth
\newif\ifXKV@st
\newif\ifXKV@sg
\newif\ifXKV@pl
\newif\ifXKV@knf
\newif\ifXKV@rkv
\newif\ifXKV@inpox
\newif\ifXKV@preset
\let\XKV@rm\@empty
\ifx\ProvidesFile\@undefined
  \message{2014/12/03 v2.7a key=value parser (HA)}
  \input xkvtxhdr
\else
  \ProvidesFile{xkeyval.tex}[2014/12/03 v2.7a key=value parser (HA)]
  \@addtofilelist{xkeyval.tex}
\fi
\def\XKV@warn#1{\message{xkeyval warning: #1}}
\def\XKV@err#1{\errmessage{xkeyval error: #1}}
\def\KV@errx{\XKV@err}
\let\KV@err\KV@errx
\def\XKV@ifstar#1{\@ifnextcharacter*{\@firstoftwo{#1}}}
\def\XKV@ifplus#1{\@ifnextcharacter+{\@firstoftwo{#1}}}
\def\XKV@makepf#1{%
  \KV@@sp@def\XKV@prefix{#1}%
  \def\XKV@resa{XKV}%
  \ifx\XKV@prefix\XKV@resa
    \XKV@err{`XKV' prefix is not allowed}%
    \let\XKV@prefix\@empty
  \else
    \edef\XKV@prefix{\ifx\XKV@prefix\@empty\else\XKV@prefix @\fi}%
  \fi
}
\def\XKV@makehd#1{%
  \expandafter\KV@@sp@def\expandafter\XKV@header\expandafter{#1}%
  \edef\XKV@header{%
    \XKV@prefix\ifx\XKV@header\@empty\else\XKV@header @\fi
  }%
}
\def\XKV@srstate#1#2{%
  \ifx\@empty#2\@empty\advance\XKV@depth\@ne\fi
  \XKV@for@n{XKV@prefix,XKV@fams,XKV@tkey,XKV@na,%
    ifXKV@st,ifXKV@pl,ifXKV@knf,CurrentOption}\XKV@resa{%
    \expandafter\let\csname\XKV@resa#1\expandafter
      \endcsname\csname\XKV@resa#2\endcsname
  }%
  \ifx\@empty#1\@empty\advance\XKV@depth\m@ne\fi
}
\def\XKV@testopta#1{%
  \XKV@ifstar{\XKV@sttrue\XKV@t@stopta{#1}}%
    {\XKV@stfalse\XKV@t@stopta{#1}}%
}
\def\XKV@t@stopta#1{\XKV@ifplus{\XKV@pltrue#1}{\XKV@plfalse#1}}
\def\XKV@testoptb#1{\@testopt{\XKV@t@stoptb#1}{KV}}
\def\XKV@t@stoptb#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@makehd{#3}%
  \KV@@sp@def\XKV@tfam{#3}%
  #1%
}
\def\XKV@testoptc#1{\@testopt{\XKV@t@stoptc#1}{KV}}
\def\XKV@t@stoptc#1[#2]#3{%
  \XKV@makepf{#2}%
  \XKV@checksanitizeb{#3}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \@testopt#1{}%
}
\def\XKV@testoptd#1#2{%
  \XKV@testoptb{%
    \edef\XKV@tempa{#2\XKV@header}%
    \def\XKV@tempb{\@testopt{\XKV@t@stoptd#1}}%
    \expandafter\XKV@tempb\expandafter{\XKV@tempa}%
  }%
}
\def\XKV@t@stoptd#1[#2]#3{%
  \@ifnextchar[{\XKV@sttrue#1{#2}{#3}}{\XKV@stfalse#1{#2}{#3}[]}%
}
\def\XKV@ifcmd#1#2#3{%
  \def\XKV@@ifcmd##1#2##2##3\@nil##4{%
    \def##4{##2}\ifx##4\@nnil
      \def##4{##1}\expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }%
  \XKV@@ifcmd#1#2{\@nil}\@nil#3%
}
\def\XKV@getkeyname#1#2{\expandafter\XKV@g@tkeyname#1=\@nil#2}
\long\def\XKV@g@tkeyname#1=#2\@nil#3{%
  \XKV@ifcmd{#1}\savevalue#3{\XKV@rkvtrue\XKV@sgfalse}{%
    \XKV@ifcmd{#1}\gsavevalue#3%
      {\XKV@rkvtrue\XKV@sgtrue}{\XKV@rkvfalse\XKV@sgfalse}%
  }%
}
\def\XKV@getsg#1#2{%
  \expandafter\XKV@ifcmd\expandafter{#1}\global#2\XKV@sgtrue\XKV@sgfalse
}
\def\XKV@define@default#1#2{%
  \expandafter\def\csname\XKV@header#1@default\expandafter
    \endcsname\expandafter{\csname\XKV@header#1\endcsname{#2}}%
}
\def\define@key{\XKV@testoptb\XKV@define@key}
\def\XKV@define@key#1{%
  \@ifnextchar[{\XKV@d@fine@k@y{#1}}{%
    \long\expandafter\def\csname\XKV@header#1\endcsname####1%
  }%
}
\def\XKV@d@fine@k@y#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \expandafter\def\csname\XKV@header#1\endcsname##1%
}
\def\define@cmdkey{\XKV@testoptd\XKV@define@cmdkey{cmd}}
\def\XKV@define@cmdkey#1#2[#3]#4{%
  \ifXKV@st\XKV@define@default{#2}{#3}\fi
  \def\XKV@tempa{\expandafter\def\csname\XKV@header#2\endcsname####1}%
  \begingroup\expandafter\endgroup\expandafter\XKV@tempa\expandafter
    {\expandafter\def\csname#1#2\endcsname{##1}#4}%
}
\def\define@cmdkeys{\XKV@testoptd\XKV@define@cmdkeys{cmd}}
\def\XKV@define@cmdkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \edef\XKV@tempa{\noexpand\XKV@define@cmdkey{#1}{\XKV@tempa}}%
    \XKV@tempa[#3]{}%
  }%
}
\def\define@choicekey{\XKV@testopta{\XKV@testoptb\XKV@define@choicekey}}
\def\XKV@define@choicekey#1{\@testopt{\XKV@d@fine@choicekey{#1}}{}}
\def\XKV@d@fine@choicekey#1[#2]#3{%
  \toks@{#2}%
  \XKV@sp@deflist\XKV@tempa{#3}\XKV@toks\expandafter{\XKV@tempa}%
  \@ifnextchar[{\XKV@d@fine@ch@icekey{#1}}{\XKV@d@fine@ch@ic@key{#1}}%
}
\def\XKV@d@fine@ch@icekey#1[#2]{%
  \XKV@define@default{#1}{#2}%
  \XKV@d@fine@ch@ic@key{#1}%
}
\def\XKV@d@fine@ch@ic@key#1{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@ch@ic@k@y
  \else\XKV@afterfi
    \expandafter\XKV@d@f@ne@ch@ic@key
  \fi
  \csname\XKV@header#1\endcsname
}
\def\XKV@d@f@ne@ch@ic@key#1#2{\XKV@d@f@n@@ch@ic@k@y#1{{#2}}}
\def\XKV@d@f@ne@ch@ic@k@y#1#2#3{\XKV@d@f@n@@ch@ic@k@y#1{{#2}{#3}}}
\def\XKV@d@f@n@@ch@ic@k@y#1#2{%
  \edef#1##1{%
    \ifXKV@st\noexpand\XKV@sttrue\else\noexpand\XKV@stfalse\fi
    \ifXKV@pl\noexpand\XKV@pltrue\else\noexpand\XKV@plfalse\fi
    \noexpand\XKV@checkchoice[\the\toks@]{##1}{\the\XKV@toks}%
  }%
  \def\XKV@tempa{\def#1####1}%
  \expandafter\XKV@tempa\expandafter{#1{##1}#2}%
}
\def\define@boolkey{\XKV@t@stopta{\XKV@testoptd\XKV@define@boolkey{}}}
\def\XKV@define@boolkey#1#2[#3]{%
  \ifXKV@pl\XKV@afterelsefi
    \expandafter\XKV@d@f@ne@boolkey
  \else\XKV@afterfi
    \expandafter\XKV@d@fine@boolkey
  \fi
  \csname\XKV@header#2\endcsname{#2}{#1#2}{#3}%
}
\def\XKV@d@fine@boolkey#1#2#3#4#5{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}}%
}
\def\XKV@d@f@ne@boolkey#1#2#3#4#5#6{%
  \XKV@d@f@ne@b@olkey#1{#2}{#3}{#4}%
    {{\csname#3\XKV@resa\endcsname#5}{#6}}%
}
\def\XKV@d@f@ne@b@olkey#1#2#3#4#5{%
  \expandafter\newif\csname if#3\endcsname
  \ifXKV@st\XKV@define@default{#2}{#4}\fi
  \ifXKV@pl
    \def#1##1{\XKV@pltrue\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \else
    \def#1##1{\XKV@plfalse\XKV@sttrue
      \XKV@checkchoice[\XKV@resa]{##1}{true,false}#5%
    }%
  \fi
}
\def\define@boolkeys{\XKV@plfalse\XKV@testoptd\XKV@define@boolkeys{}}
\def\XKV@define@boolkeys#1#2[#3]{%
  \XKV@sp@deflist\XKV@tempa{#2}%
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \expandafter\XKV@d@fine@boolkeys\expandafter{\XKV@tempa}{#1}{#3}%
  }%
}
\def\XKV@d@fine@boolkeys#1#2#3{%
  \expandafter\XKV@d@f@ne@b@olkey\csname\XKV@header#1\endcsname
    {#1}{#2#1}{#3}{{\csname#2#1\XKV@resa\endcsname}}%
}
\def\XKV@cc{\XKV@testopta{\@testopt\XKV@checkchoice{}}}
\def\XKV@checkchoice[#1]#2#3{%
  \def\XKV@tempa{#1}%
  \ifXKV@st\lowercase{\fi
  \ifx\XKV@tempa\@empty
    \def\XKV@tempa{\XKV@ch@ckch@ice\@nil{#2}{#3}}%
  \else
    \def\XKV@tempa{\XKV@ch@ckchoice#1\@nil{#2}{#3}}%
  \fi
  \ifXKV@st}\fi\XKV@tempa
}
\def\XKV@ch@ckchoice#1#2\@nil#3#4{%
  \def\XKV@tempa{#2}%
  \ifx\XKV@tempa\@empty\XKV@afterelsefi
    \XKV@ch@ckch@ice#1{#3}{#4}%
  \else\XKV@afterfi
    \XKV@@ch@ckchoice#1#2{#3}{#4}%
  \fi
}
\def\XKV@ch@ckch@ice#1#2#3{%
  \def\XKV@tempa{#1}%
  \ifx\XKV@tempa\@nnil\let\XKV@tempa\@empty\else
    \def\XKV@tempa{\def#1{#2}}%
  \fi
  \in@{,#2,}{,#3,}%
  \ifin@
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@firstoftwo
    \else
      \XKV@addtomacro@n\XKV@tempa\@firstofone
    \fi
  \else
    \ifXKV@pl
      \XKV@addtomacro@n\XKV@tempa\@secondoftwo
    \else
      \XKV@toks{#2}%
      \XKV@err{value `\the\XKV@toks' is not allowed}%
      \XKV@addtomacro@n\XKV@tempa\@gobble
    \fi
  \fi
  \XKV@tempa
}
\def\XKV@@ch@ckchoice#1#2#3#4{%
  \edef\XKV@tempa{\the\count@}\count@\z@
  \def\XKV@tempb{#3}%
  \def\XKV@tempc##1,{%
    \def#1{##1}%
    \ifx#1\@nnil
      \def#1{#3}\def#2{-1}\count@\XKV@tempa
      \ifXKV@pl
        \let\XKV@tempd\@secondoftwo
      \else
        \XKV@toks{#3}%
        \XKV@err{value `\the\XKV@toks' is not allowed}%
        \let\XKV@tempd\@gobble
      \fi
    \else
      \ifx#1\XKV@tempb
        \edef#2{\the\count@}\count@\XKV@tempa
        \ifXKV@pl
          \let\XKV@tempd\XKV@@ch@ckch@ice
        \else
          \let\XKV@tempd\XKV@@ch@ckch@ic@
        \fi
      \else
        \advance\count@\@ne
        \let\XKV@tempd\XKV@tempc
      \fi
    \fi
    \XKV@tempd
  }%
  \XKV@tempc#4,\@nil,%
}
\def\XKV@@ch@ckch@ice#1\@nil,{\@firstoftwo}
\def\XKV@@ch@ckch@ic@#1\@nil,{\@firstofone}
\def\key@ifundefined{\@testopt\XKV@key@ifundefined{KV}}
\def\XKV@key@ifundefined[#1]#2{%
  \XKV@makepf{#1}%
  \XKV@checksanitizeb{#2}\XKV@fams
  \expandafter\XKV@sp@deflist\expandafter
    \XKV@fams\expandafter{\XKV@fams}%
  \XKV@key@if@ndefined
}
\def\XKV@key@if@ndefined#1{%
  \XKV@knftrue
  \KV@@sp@def\XKV@tkey{#1}%
  \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{\XKV@header\XKV@tkey}{}{\XKV@knffalse}%
  }%
  \ifXKV@knf
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
}
\def\disable@keys{\XKV@testoptb\XKV@disable@keys}
\def\XKV@disable@keys#1{%
  \XKV@checksanitizeb{#1}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@ifundefined{\XKV@header\XKV@tempa}{%
      \XKV@err{key `\XKV@tempa' undefined}%
    }{%
      \edef\XKV@tempb{%
        \noexpand\XKV@warn{key `\XKV@tempa' has been disabled}%
      }%
      \XKV@ifundefined{\XKV@header\XKV@tempa @default}{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}}%
      }{%
        \edef\XKV@tempc{\noexpand\XKV@define@key{\XKV@tempa}[]}%
      }%
      \expandafter\XKV@tempc\expandafter{\XKV@tempb}%
    }%
  }%
}
\def\presetkeys{\XKV@stfalse\XKV@testoptb\XKV@presetkeys}
\def\gpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@presetkeys}
\def\XKV@presetkeys#1#2{%
  \XKV@pr@setkeys{#1}{preseth}%
  \XKV@pr@setkeys{#2}{presett}%
}
\def\XKV@pr@setkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@checksanitizea{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname
      XKV@\XKV@header#2\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\delpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@delpresetkeys}
\def\gdelpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@delpresetkeys}
\def\XKV@delpresetkeys#1#2{%
  \XKV@d@lpresetkeys{#1}{preseth}%
  \XKV@d@lpresetkeys{#2}{presett}%
}
\def\XKV@d@lpresetkeys#1#2{%
  \XKV@ifundefined{XKV@\XKV@header#2}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      #2\endcsname{#1}\XKV@getkeyname
  }%
}
\def\unpresetkeys{\XKV@stfalse\XKV@testoptb\XKV@unpresetkeys}
\def\gunpresetkeys{\XKV@sttrue\XKV@testoptb\XKV@unpresetkeys}
\def\XKV@unpresetkeys{%
  \XKV@ifundefined{XKV@\XKV@header preseth}{%
    \XKV@err{no presets defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header preseth\endcsname\@undefined
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header presett\endcsname\@undefined
  }%
}
\def\savekeys{\XKV@stfalse\XKV@testoptb\XKV@savekeys}
\def\gsavekeys{\XKV@sttrue\XKV@testoptb\XKV@savekeys}
\def\XKV@savekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@checksanitizeb{#1}\XKV@tempa
    \ifXKV@st\expandafter\global\fi\expandafter\def\csname XKV@%
      \XKV@header save\expandafter\endcsname\expandafter{\XKV@tempa}%
  }{%
    \expandafter\XKV@merge\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\delsavekeys{\XKV@stfalse\XKV@testoptb\XKV@delsavekeys}
\def\gdelsavekeys{\XKV@sttrue\XKV@testoptb\XKV@delsavekeys}
\def\XKV@delsavekeys#1{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \expandafter\XKV@delete\csname XKV@\XKV@header
      save\endcsname{#1}\XKV@getsg
  }%
}
\def\unsavekeys{\XKV@stfalse\XKV@testoptb\XKV@unsavekeys}
\def\gunsavekeys{\XKV@sttrue\XKV@testoptb\XKV@unsavekeys}
\def\XKV@unsavekeys{%
  \XKV@ifundefined{XKV@\XKV@header save}{%
    \XKV@err{no save keys defined for `\XKV@header'}%
  }{%
    \ifXKV@st\expandafter\global\fi\expandafter\let
      \csname XKV@\XKV@header save\endcsname\@undefined
  }%
}
\def\setkeys{\XKV@testopta{\XKV@testoptc\XKV@setkeys}}
\long\def\XKV@setkeys[#1]#2{%
  \XKV@checksanitizea{#2}\XKV@resb
  \let\XKV@naa\@empty
  \XKV@for@o\XKV@resb\XKV@tempa{%
    \expandafter\XKV@g@tkeyname\XKV@tempa=\@nil\XKV@tempa
    \XKV@addtolist@x\XKV@naa\XKV@tempa
  }%
  \ifnum\XKV@depth=\z@\let\XKV@rm\@empty\fi
  \XKV@usepresetkeys{#1}{preseth}%
  \expandafter\XKV@s@tkeys\expandafter{\XKV@resb}{#1}%
  \XKV@usepresetkeys{#1}{presett}%
  \let\CurrentOption\@empty
}
\def\XKV@usepresetkeys#1#2{%
  \XKV@presettrue
  \XKV@for@eo\XKV@fams\XKV@tfam{%
    \XKV@makehd\XKV@tfam
    \XKV@ifundefined{XKV@\XKV@header#2}{}{%
      \XKV@toks\expandafter\expandafter\expandafter
        {\csname XKV@\XKV@header#2\endcsname}%
      \@expandtwoargs\XKV@s@tkeys{\the\XKV@toks}%
        {\XKV@naa\ifx\XKV@naa\@empty\else,\fi#1}%
    }%
  }%
  \XKV@presetfalse
}
\long\def\XKV@s@tkeys#1#2{%
  \XKV@sp@deflist\XKV@na{#2}%
  \XKV@for@n{#1}\CurrentOption{%
    \expandafter\XKV@s@tk@ys\CurrentOption==\@nil
  }%
}
\long\def\XKV@s@tk@ys#1=#2=#3\@nil{%
  \XKV@g@tkeyname#1=\@nil\XKV@tkey
  \expandafter\KV@@sp@def\expandafter\XKV@tkey\expandafter{\XKV@tkey}%
  \ifx\XKV@tkey\@empty
    \XKV@toks{#2}%
    \ifcat$\the\XKV@toks$\else
      \XKV@err{no key specified for value `\the\XKV@toks'}%
    \fi
  \else
    \@expandtwoargs\in@{,\XKV@tkey,}{,\XKV@na,}%
    \ifin@\else
      \XKV@knftrue
      \KV@@sp@def\XKV@tempa{#2}%
      \ifXKV@preset\XKV@s@tk@ys@{#3}\else
        \ifXKV@pl
          \XKV@for@eo\XKV@fams\XKV@tfam{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \else
          \XKV@whilist\XKV@fams\XKV@tfam\ifXKV@knf\fi{%
            \XKV@makehd\XKV@tfam
            \XKV@s@tk@ys@{#3}%
          }%
        \fi
      \fi
      \ifXKV@knf
        \ifXKV@inpox
          \ifx\XKV@doxs\relax
            \ifx\@currext\@clsextension\else
              \let\CurrentOption\XKV@tkey\@unknownoptionerror
            \fi
          \else\XKV@doxs\fi
        \else
          \ifXKV@st
            \XKV@addtolist@o\XKV@rm\CurrentOption
          \else
            \XKV@err{`\XKV@tkey' undefined in families `\XKV@fams'}%
          \fi
        \fi
      \else
        \ifXKV@inpox\ifx\XKV@testclass\XKV@documentclass
          \expandafter\XKV@useoption\expandafter{\CurrentOption}%
        \fi\fi
      \fi
    \fi
  \fi
}
\def\XKV@s@tk@ys@#1{%
  \XKV@ifundefined{\XKV@header\XKV@tkey}{}{%
    \XKV@knffalse
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter{\XKV@tempa}%
    \ifx\@empty#1\@empty\XKV@afterelsefi
      \XKV@ifundefined{\XKV@header\XKV@tkey @default}{%
        \XKV@err{no value specified for key `\XKV@tkey'}%
      }{%
        \expandafter\expandafter\expandafter\XKV@default
          \csname\XKV@header\XKV@tkey @default\endcsname\@nil
      }%
    \else\XKV@afterfi
      \XKV@srstate{@\romannumeral\XKV@depth}{}%
      \csname\XKV@header\XKV@tkey\expandafter
        \endcsname\expandafter{\XKV@tempa}\relax
      \XKV@srstate{}{@\romannumeral\XKV@depth}%
    \fi
  }%
}
\def\XKV@testsavekey#1#2{%
  \ifXKV@rkv\else
    \XKV@for@o#1\XKV@resa{%
      \expandafter\XKV@ifcmd\expandafter{\XKV@resa}\global\XKV@resa{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgtrue
        \fi
      }{%
        \ifx#2\XKV@resa
          \XKV@rkvtrue\XKV@sgfalse
        \fi
      }%
    }%
  \fi
}
\long\def\XKV@replacepointers#1{%
  \let\XKV@tempa\@empty
  \let\XKV@resa\@empty
  \XKV@r@placepointers#1\usevalue\@nil
}
\long\def\XKV@r@placepointers#1\usevalue#2{%
  \XKV@addtomacro@n\XKV@tempa{#1}%
  \def\XKV@tempb{#2}%
  \ifx\XKV@tempb\@nnil\else\XKV@afterfi
    \XKV@ifundefined{XKV@\XKV@header#2@value}{%
      \XKV@err{no value recorded for key `#2'; ignored}%
      \XKV@r@placepointers
    }{%
      \@expandtwoargs\in@{,#2,}{,\XKV@resa,}%
      \ifin@\XKV@afterelsefi
        \XKV@err{back linking pointers; pointer replacement canceled}%
      \else\XKV@afterfi
        \XKV@addtolist@x\XKV@resa{#2}%
        \expandafter\expandafter\expandafter\XKV@r@placepointers
          \csname XKV@\XKV@header#2@value\endcsname
      \fi
    }%
  \fi
}
\def\XKV@default#1#2\@nil{%
  \expandafter\edef\expandafter\XKV@tempa
    \expandafter{\expandafter\@gobble\string#1}%
  \edef\XKV@tempb{\XKV@header\XKV@tkey}%
  \@onelevel@sanitize\XKV@tempb
  \ifx\XKV@tempa\XKV@tempb
    \begingroup
      \expandafter\def\csname\XKV@header\XKV@tkey\endcsname##1{%
        \gdef\XKV@tempa{##1}%
      }%
      \csname\XKV@header\XKV@tkey @default\endcsname
    \endgroup
    \XKV@ifundefined{XKV@\XKV@header save}{}{%
      \expandafter\XKV@testsavekey\csname XKV@\XKV@header
        save\endcsname\XKV@tkey
    }%
    \ifXKV@rkv
      \ifXKV@sg\expandafter\global\fi\expandafter\let
        \csname XKV@\XKV@header\XKV@tkey @value\endcsname\XKV@tempa
    \fi
    \expandafter\XKV@replacepointers\expandafter
      {\XKV@tempa}\XKV@afterelsefi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \expandafter#1\expandafter{\XKV@tempa}\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \else\XKV@afterfi
    \XKV@srstate{@\romannumeral\XKV@depth}{}%
    \csname\XKV@header\XKV@tkey @default\endcsname\relax
    \XKV@srstate{}{@\romannumeral\XKV@depth}%
  \fi
}
\def\setrmkeys{\XKV@testopta{\XKV@testoptc\XKV@setrmkeys}}
\def\XKV@setrmkeys[#1]{%
  \def\XKV@tempa{\XKV@setkeys[#1]}%
  \expandafter\XKV@tempa\expandafter{\XKV@rm}%
}
\XKVcatcodes
\endinput
%%
%% End of file `xkeyval.tex'.


==> xkvutils.tex <==
%%
%% This is file `xkvutils.tex',
%% generated with the docstrip utility.
%%
%% The original source files were:
%%
%% xkeyval.dtx  (with options: `xkvutils')
%% 
%% ---------------------------------------
%% Copyright (C) 2004-2014 Hendri Adriaens
%% ---------------------------------------
%%
%% This work may be distributed and/or modified under the
%% conditions of the LaTeX Project Public License, either version 1.3
%% of this license or (at your option) any later version.
%% The latest version of this license is in
%%   http://www.latex-project.org/lppl.txt
%% and version 1.3 or later is part of all distributions of LaTeX
%% version 2003/12/01 or later.
%%
%% This work has the LPPL maintenance status "maintained".
%%
%% This Current Maintainer of this work is Hendri Adriaens.
%%
%% This work consists of the file xkeyval.dtx and derived files
%% keyval.tex, xkvtxhdr.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvutils.tex, pst-xkey.tex, pst-xkey.sty, xkveca.cls,
%% xkvecb.cls, xkvesa.sty, xkvesb.sty, xkvesc.sty, xkvex1.tex,
%% xkvex2.tex, xkvex3.tex and xkvex4.tex.
%%
%% The following files constitute the xkeyval bundle and must be
%% distributed as a whole: readme, xkeyval.pdf, keyval.tex,
%% pst-xkey.sty, pst-xkey.tex, xkeyval.sty, xkeyval.tex, xkvview.sty,
%% xkvltxp.sty, xkvtxhdr.tex, xkvutils.tex, pst-xkey.dtx and xkeyval.dtx.
%%
\csname XKeyValUtilsLoaded\endcsname
\let\XKeyValUtilsLoaded\endinput
\edef\XKeyValUtilsCatcodes{%
  \catcode`\noexpand\@\the\catcode`\@\relax
  \let\noexpand\XKeyValUtilsCatcodes\relax
}
\catcode`\@=11\relax
\newtoks\XKV@toks
\newtoks\XKV@tempa@toks
\long\def\@firstoftwo#1#2{#1}
\long\def\@secondoftwo#1#2{#2}
\long\def\XKV@afterfi#1\fi{\fi#1}
\long\def\XKV@afterelsefi#1\else#2\fi{\fi#1}
\ifx\ifcsname\@undefined\XKV@afterelsefi
  \def\XKV@ifundefined#1{%
    \begingroup\expandafter\expandafter\expandafter\endgroup
      \expandafter\ifx\csname#1\endcsname\relax
      \expandafter\@firstoftwo
    \else
      \expandafter\@secondoftwo
    \fi
  }
\else
  \def\XKV@ifundefined#1{%
    \ifcsname#1\endcsname
      \expandafter\@secondoftwo
    \else
      \expandafter\@firstoftwo
    \fi
  }
\fi
\XKV@ifundefined{ver@keyval.sty}{
  \input keyval
  \expandafter\def\csname ver@keyval.sty\endcsname{1999/03/16}
}{}
\long\def\@ifnextcharacter#1#2#3{%
  \@ifnextchar\bgroup
  {\@ifnextchar{#1}{#2}{#3}}%
  {\@ifncharacter{#1}{#2}{#3}}%
}
\long\def\@ifncharacter#1#2#3#4{%
  \if\string#1\string#4%
    \expandafter\@firstoftwo
  \else
    \expandafter\@secondoftwo
  \fi
  {#2}{#3}#4%
}
\long\def\XKV@for@n#1#2#3{%
  \XKV@tempa@toks{#1}\edef#2{\the\XKV@tempa@toks}%
  \ifx#2\@empty
    \XKV@for@break
  \else
    \expandafter\XKV@f@r
  \fi
  #2{#3}#1,\@nil,%
}
\long\def\XKV@f@r#1#2#3,{%
  \XKV@tempa@toks{#3}\edef#1{\the\XKV@tempa@toks}%
  \ifx#1\@nnil
    \expandafter\@gobbletwo
  \else
    #2\expandafter\XKV@f@r
  \fi
  #1{#2}%
}
\long\def\XKV@for@break #1\@nil,{\fi}
\long\def\XKV@for@o#1{\expandafter\XKV@for@n\expandafter{#1}}
\long\def\XKV@for@en#1#2#3{\XKV@f@r#2{#3}#1,\@nil,}
\long\def\XKV@for@eo#1#2#3{%
  \def#2{\XKV@f@r#2{#3}}\expandafter#2#1,\@nil,%
}
\long\def\XKV@whilist#1#2#3\fi#4{%
  #3\expandafter\XKV@wh@list#1,\@nil,\@nil\@@#2#3\fi{#4}{}\fi
}
\long\def\XKV@wh@list#1,#2\@@#3#4\fi#5#6{%
  \def#3{#1}%
  \ifx#3\@nnil
    \def#3{#6}\expandafter\XKV@wh@l@st
  \else
    #4%
      #5\expandafter\expandafter\expandafter\XKV@wh@list
    \else
      \def#3{#6}\expandafter\expandafter\expandafter\XKV@wh@l@st
    \fi
  \fi
  #2\@@#3#4\fi{#5}{#1}%
}
\long\def\XKV@wh@l@st#1\@@#2#3\fi#4#5{}
\long\def\XKV@addtomacro@n#1#2{%
  \XKV@tempa@toks\expandafter{#1#2}%
  \edef#1{\the\XKV@tempa@toks}%
}
\def\XKV@addtomacro@o#1#2{%
  \expandafter\XKV@addtomacro@n\expandafter#1\expandafter{#2}%
}
\def\XKV@addtolist@n#1#2{%
  \ifx#1\@empty
    \XKV@addtomacro@n#1{#2}%
  \else
    \XKV@addtomacro@n#1{,#2}%
  \fi
}
\def\XKV@addtolist@o#1#2{%
  \ifx#1\@empty
    \XKV@addtomacro@o#1#2%
  \else
    \XKV@addtomacro@o#1{\expandafter,#2}%
  \fi
}
\def\XKV@addtolist@x#1#2{\edef#1{#1\ifx#1\@empty\else,\fi#2}}
\def\@selective@sanitize{\@testopt\@s@lective@sanitize\@M}
\def\@s@lective@sanitize[#1]#2#3{%
  \begingroup
    \count@#1\relax\advance\count@\@ne
    \XKV@toks\expandafter{#3}%
    \def#3{#2}\@onelevel@sanitize#3%
    \edef#3{{#3}{\the\XKV@toks}}%
    \expandafter\@s@l@ctive@sanitize\expandafter#3#3%
    \expandafter\XKV@tempa@toks\expandafter{#3}%
  \expandafter\endgroup\expandafter\toks@\expandafter{\the\XKV@tempa@toks}%
  \edef#3{\the\toks@}%
}
\def\@s@l@ctive@sanitize#1#2#3{%
  \def\@i{\futurelet\@@tok\@ii}%
  \def\@ii{%
    \expandafter\@iii\meaning\@@tok\relax
    \ifx\@@tok\@s@l@ctive@sanitize
      \let\@@cmd\@gobble
    \else
      \ifx\@@tok\@sptoken
        \XKV@toks\expandafter{#1}\edef#1{\the\XKV@toks\space}%
        \def\@@cmd{\afterassignment\@i\let\@@tok= }%
      \else
        \let\@@cmd\@iv
      \fi
    \fi
    \@@cmd
  }%
  \def\@iii##1##2\relax{\if##1\@backslashchar\let\@@tok\relax\fi}%
  \def\@iv##1{%
    \toks@\expandafter{#1}\XKV@toks{##1}%
    \ifx\@@tok\bgroup
      \advance\count@\m@ne
      \ifnum\count@>\z@
        \begingroup
          \def#1{\expandafter\@s@l@ctive@sanitize
            \csname\string#1\endcsname{#2}}%
          \expandafter#1\expandafter{\the\XKV@toks}%
          \XKV@toks\expandafter\expandafter\expandafter
            {\csname\string#1\endcsname}%
          \edef#1{\noexpand\XKV@toks{\the\XKV@toks}}%
        \expandafter\endgroup#1%
      \fi
      \edef#1{\the\toks@{\the\XKV@toks}}%
      \advance\count@\@ne
      \let\@@cmd\@i
    \else
      \edef#1{\expandafter\string\the\XKV@toks}%
      \expandafter\in@\expandafter{#1}{#2}%
      \edef#1{\the\toks@\ifin@#1\else
              \ifx\@@tok\@sptoken\space\else\the\XKV@toks\fi\fi}%
      \edef\@@cmd{\noexpand\@i\ifx\@@tok\@sptoken\the\XKV@toks\fi}%
    \fi
    \@@cmd
  }%
  \let#1\@empty\@i#3\@s@l@ctive@sanitize
}
\long\def\XKV@checksanitizea#1#2{%
  \XKV@ch@cksanitize{#1}#2=%
  \ifin@\else\XKV@ch@cksanitize{#1}#2,\fi
  \ifin@\@selective@sanitize[0]{,=}#2\fi
}
\def\XKV@checksanitizeb#1#2{%
  \XKV@ch@cksanitize{#1}#2,%
  \ifin@\@selective@sanitize[0],#2\fi
}
\long\def\XKV@ch@cksanitize#1#2#3{%
  \XKV@tempa@toks{#1}\edef#2{\the\XKV@tempa@toks}%
  \@onelevel@sanitize#2%
  \@expandtwoargs\in@#3{#2}%
  \ifin@
    \long\def#2##1#3##2\@nil{%
      \XKV@tempa@toks{##2}\edef#2{\the\XKV@tempa@toks}%
      \ifx#2\@empty\else\in@false\fi
    }%
    #2#1#3\@nil
  \fi
  \XKV@tempa@toks{#1}\edef#2{\the\XKV@tempa@toks}%
}
\def\XKV@sp@deflist#1#2{%
  \let#1\@empty
  \XKV@for@n{#2}\XKV@resa{%
    \expandafter\KV@@sp@def\expandafter\XKV@resa\expandafter{\XKV@resa}%
    \XKV@addtomacro@o#1{\expandafter,\XKV@resa}%
  }%
  \ifx#1\@empty\else
    \def\XKV@resa,##1\@nil{\def#1{##1}}%
    \expandafter\XKV@resa#1\@nil
  \fi
}
\def\XKV@merge#1#2#3{%
  \XKV@checksanitizea{#2}\XKV@tempa
  \XKV@for@o\XKV@tempa\XKV@tempa{%
    \XKV@pltrue
    #3\XKV@tempa\XKV@tempb
    \let\XKV@tempc#1%
    \let#1\@empty
    \XKV@for@o\XKV@tempc\XKV@tempc{%
      #3\XKV@tempc\XKV@tempd
      \ifx\XKV@tempb\XKV@tempd
        \XKV@plfalse
        \XKV@addtolist@o#1\XKV@tempa
      \else
        \XKV@addtolist@o#1\XKV@tempc
      \fi
    }%
    \ifXKV@pl\XKV@addtolist@o#1\XKV@tempa\fi
  }%
  \ifXKV@st\global\let#1#1\fi
}
\def\XKV@delete#1#2#3{%
  \XKV@checksanitizeb{#2}\XKV@tempa
  \let\XKV@tempb#1%
  \let#1\@empty
  \XKV@for@o\XKV@tempb\XKV@tempb{%
    #3\XKV@tempb\XKV@tempc
    \@expandtwoargs\in@{,\XKV@tempc,}{,\XKV@tempa,}%
    \ifin@\else\XKV@addtolist@o#1\XKV@tempb\fi
  }%
  \ifXKV@st\global\let#1#1\fi
}
\XKeyValUtilsCatcodes
\endinput
%%
%% End of file `xkvutils.tex'.

